Experimental measurement of the vorticity-strain alignment around extreme energy transfer events

This work experimentally explores the alignment of the vorticity vector and the strain-rate tensor eigenvectors at locations of extreme upscale and downscale energy transfer. We show that the turbulent von Karman flow displays vorticity-strain alignment behavior across a large range of Reynolds numbers, which are very similar to previous studies on homogeneous, isotropic turbulence. We observe that this behavior is amplified for the largest downscale energy transfer events, which tend to be associated with sheet-like geometries. These events are also shown to have characteristics previously associated with high flow field non-linearity and singularities. In contrast the largest upscale energy transfer events display much different structures which showcase a strong preference for vortex-compression. We then show further evidence to the argument that strain-self-amplification is the most salient feature in characterizing cascade direction. Finally, we identify possible invariant behavior for the largest energy transfer events, even at scales near the Kolmogorov scale.

==> sections/acknowledge.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Acknowledgment} \label{sec:acknow}

We gratefully acknowledge support from:
ANR Exploit
BANG
CNRS
Marie Curie
The authors also greatly thank Mauro Abella for his freight elevator rescue and enjoyable lunchtime discussions. 


MAJOR TAKEAWAYS:
-structure at lowest energy levels, not all unifrom distributed
- vorticity vector preference for perpendicularity with the largest strain eigen vector in both up and down scale energy trasnfer
- down scale make sheets
- strain self amp is what mainly differnetiates the two directions 
- inconsistency with nonlinearities (large downscale is more 2D, it less non linearity) but it also crowds farther alone vielfosse line, where there is more nonlinearity
-vortex compression plays major role in upscale energy trasfer
-extensive eig vectors in downscale are similar magnitude
-in upscale enrgy transger intermediate is much smaller compared to the other two
-regions of inverse or direct cascade had more distinct differences in strain-rate differences than vorticity, as events in positive and negative enstrophy QR space existed in both cascade directions. 
$\overline{\Pi_{\vee}}$
$\overline{\mathcal{D}_{\vee}}$
